Ditto: An Elastic and Adaptive Memory-Disaggregated Caching System

In-memory caching systems are fundamental building blocks in cloud services. However, due to the coupled CPU and memory on monolithic servers, existing caching systems cannot elastically adjust resources in a resource-efficient and agile manner. To achieve better elasticity, we propose to port in-memory caching systems to the disaggregated memory (DM) architecture, where compute and memory resources are decoupled and can be allocated flexibly. However, constructing an elastic caching system on DM is challenging since accessing cached objects with CPU-bypass remote memory accesses hinders the execution of caching algorithms. Moreover, the elastic changes of compute and memory resources on DM affect the access patterns of cached data, compromising the hit rates of caching algorithms. We design Ditto, the first caching system on DM, to address these challenges. Ditto first proposes a client-centric caching framework to efficiently execute various caching algorithms in the compute pool of DM, relying only on remote memory accesses. Then, Ditto employs a distributed adaptive caching scheme that adaptively switches to the best-fit caching algorithm in real-time based on the performance of multiple caching algorithms to improve cache hit rates. Our experiments show that Ditto effectively adapts to the changing resources on DM and outperforms the state-of-the-art caching systems by up to 3.6x in real-world workloads and 9x in YCSB

==> osdi-rebuttal.tex <==
Thanks for the constructive comments. We address all of your questions and concerns in individual reviews.

**Why would a datacenter operator deploy machines that only have one CPU core that could never be used in the future for anything but serving RDMAs? (Reviews A, B, and C)**  
**Reply:** The one-CPU-core servers are used to simulate the weak compute power in the memory node of the disaggregated memory (DM) architecture [50,55,R1,R2]. DM decouples the compute and memory resources in monolithic servers and forms independent compute and memory resource pools. In such an architecture, compute blades run applications with a small amount of memory as runtime cache, while the memory pool stores and serves application data with high-speed interconnect like RDMA and CXL. The weak compute power on MNs is reserved only for managing memory space and network connections. Due to resource pooling and decoupled hardware deployments, DM enjoys higher resource utilization and elasticity [1,24,29,44,46,54,56]. 

**It seems like Ditto's cost for the adaptive policy is almost never worth the tradeoff. Does adding the full suite of algorithms (or at least more of them) help or hurt? (Review A)**  
**Reply:** Compared with pure sampling, conducting adaptive caching does have performance tradeoffs. The performance gain is explained as follows. On workloads that have clear preferences on eviction algorithms, users do not necessarily know the best eviction algorithm in advance. Conducting adaptive caching can effectively select the best one for the user and gain a higher hit rate than randomly selecting an inferior one (Figure 16). On workloads that change the access pattern with time, conducting adaptive caching can dynamically adapt to the best algorithm with the workload change. As a result, the overall hit rate can outperform all individual conventional caching algorithms (Figures 18 and 20).   
As for adding more algorithms for adaptive caching, previous works have investigated the effect of using more experts and found that using two complementary algorithms generates the best result [43,53]. The situation is the same for Ditto. However, the ability to integrate various algorithms is still needed since better experts can have higher hit rates. The exploration of better experts on DM is our future work.

**Motivation for flexibility in Section 3. (Reviews A and C)**  
**Reply:** In Section 3, we find that the improved elasticity of the disaggregated memory architecture exacerbates the workload change and hence urges caching algorithms to adapt to these workload changes. Elastically adding or decreasing clients and cache sizes are the benefits of DM, but they affect the hit rates of caching algorithms. First, since clients have different access patterns, adding or removing clients dynamically can change the entire workload and affect the hit rates of caching algorithms. Besides, workloads with different cache sizes may have different affinity on caching algorithms [43]. We have conducted experiments in Section 3 to show how these aspects affect the hit rates of LRU and LFU.

**Unrealistic baselines. (Reviews A and C)**  
**Reply:** Thank you for your suggestions. We will make our comparisons more realistic by 1) optimizing Precise-LRU to make it perform more reasonably, 2) comparing with CliqueMap with more CPU cores, and 3) demonstrating the elasticity benefits of the proposed memory-disaggregated caching system (Ditto) over monolithic-server-based ones. 

**Can you say a bit about how LRU-K is implemented? (Review A)**  
**Reply:** Ditto approximates LRU-K by overwriting the metadata update rules and adding an additional timestamp field for LRU-K. Specifically, for LRU-K, we maintain K 32-bit timestamp slots as an array in the slot metadata and use the *freq* field to construct a ring buffer. Each time a client accesses an object it first updates the *freq* field with RDMA\_FAA. It then updates the timestamp slot indexed by $F\text{ mod }K$, where $F$ is the return value of RDMA\_FAA. On eviction, there are two cases for the sampled objects. If $freq < K$, we evict the object if its *insert\_ts* is less than a threshold, which approximates the FIFO eviction in the access buffer. Otherwise ($freq \ge K$), we order sampled objects with the timestamp indexed by $(freq - K)\text{ mod }K$ and evict the object with the least timestamp value. Such an approach will not introduce severe metadata overhead because LRU-K is generally adopted with small Ks, *e.g.*, LRU-2 [R3]. Besides, The metadata overhead can be further mitigated by using timestamps with lower precision or overwriting the *last\_ts* field in the metadata when executed together with algorithms that don't rely on the *last\_ts* field.

**Hash table efficiency. (Review A)**  
**Reply:** The bandwidth waste is a trade-off to reduce the additional RDMA requests on sampling. Ditto is bottlenecked by the message rate of RDMA network interface cards and the overall hit rate. As shown in Figure 15, Ditto achieves maximum 6Mops throughput with 256B object sizes and 320B buckets (40B slot with 8 associativities). The consumed bandwidth is 27Gbps, which is lower than the 100Gbps bandwidth of the Connect-X 6 RNIC in our experiments. Hence, it is worthwhile to sacrifice the bandwidth to reduce an additional RDMA request.

**Does CliqueMap implementation also only use a single core to handle SET requests? Is it fair to compare Ditto since CliqueMap also handles replication and fault tolerance? (Reviews A and B)**  
**Reply:** We use one CPU core for CliqueMap to match the resource consumption of Ditto. Since there is no open-source implementation of CliqueMap, we implemented it in the same codebase as Ditto for a fair comparison. We disabled the replication and fault-tolerance of CliqueMap to focus on the cache replacement efficiency.

**Justification for the concern that low client-offered parallelism may exacerbate cache miss penalty. (Review A)**  
**Reply:** The 64-client parallelism can be justified. We have achieved more than 200 Kqps with 64 clients, while, according to Twitter's statistics, the maximum request rate among all 54 clusters is 26.40 Kqps (https://github.com/twitter/cache-trace/blob/master/stat/2020Mar.md). We can use approximately 10 clients to reach the request rate of Twitter.

**Clarifications of Figures (Review A)**  
**Reply:** The unit of y-axis of Figure 15 is microseconds. The x-axis of Figure 18a is "Throughput" and "Hit rate" respectively for each bar set.

**Why are CM-LRU and CM-LFU's hit rates worse than Ditto-LRU and Ditto-LFU in Figure 19? (Review A)**  
**Reply:** In some situations, random eviction can outperform LRU or LFU. The absolute hit rate for our LRU-friendly and LFU-friendly workloads are 0.55 and 0.37, respectively. They are selected as LRU-firendly because their LRU hit rate is higher than that of LFU, and vice versa. With the relatively low absolute hit rate, Ditto-LRU and Ditto-LFU introduce some randomization in the sampling process, and thus achieve a higher hit rate. Figure 1 of [R7] shows a similar experimental phenomenon.

**Why isn't Ditto upperbounded by max{Ditto-LRU, Ditto-LFU} in Figure 20? (Review A)**  
**Reply:** As we are using a real-world Twitter workload in the experiment, it does have some temporal access patterns that the workload alternatively switches between LRU-friendly and LFU-friendly so that Ditto can outperform both Ditto-LRU and Ditto-LFU.

**Figures 21 and 22 show the effect of different cache sizes, but were these changed at runtime? (Review C)**  
**Reply:** No. We evaluated the hit rate under each kind of cache size. 

**Horizontal scaling of the cache. (Review B)**  
**Reply:** We have discussed the problem with horizontal scaling of monolithic-server-based caching systems in Section 2.1. The performance of monolithic-server-based caching systems will be affected because their data have to be resharded according to the new configuration.

**The paper does not discuss how security is handled w.r.t. the memory pool. (Review B)**  
**Reply:** Handling security issues of the disaggregated memory pool is orthogonal to this paper. There are other related works focusing on constructing a security memory pool [R8,R9]. Ditto can leverage these approaches to construct a secure memory-disaggregated caching system.

**For a system that uses remote memory in such a tight manner, system evolution seems very difficult. (Review B)**  
**Reply:** System evolution is not difficult. It is because in our paper we design remote memory as a cache service and the application system is decoupled with the cache service. The application system can stop using the cache service, do evolution, and then reuse the cache service.

**The client-centric approach is interesting but is it general enough that one can use different algorithms easily? (Review B)**  
**Reply:** Allowing applications to easily integrate various caching algorithms in a client-centric manner is the goal of our paper. We propose a client-centric caching framework to efficiently support various caching algorithms. The generality is the same as function-based caching algorithms [40]. Besides, in our system, we decouple the caching algorithm design from the data structure design, which is similar to Hyperbolic caching and LHD [8,9]. Hence, algorithm integration is even simplified by using our system. As for the ML-based caching approaches, we propose a lightweight distributed machine learning scheme so that various integrated caching algorithms can be automatically adopted according to workload change.

**Resharding of keys is not discussed in the paper. (Review B)**  
**Reply:** This paper focuses on realizing caching algorithms on a memory-disaggregated caching system. The design of Ditto is orthogonal to the data sharding approaches on DM.

[R1]. Zhang, Ming, et al. "FORD: Fast One-sided RDMA-based Distributed Transactions for Disaggregated Persistent Memory." in FAST, 2022.  
[R2]. Li, Pengfei, et al. "ROLEX: A Scalable RDMA-oriented Learned Key-Value Store for Disaggregated Memory Systems." in FAST, 2023.  
[R3]. Montazeri, Alireza, et al. "LRU-2 vs 2-LRU: An Analytical Study." in LCN. IEEE, 2018.  
[R4]. Wei, Xingda, et al. "Fast in-memory transaction processing using RDMA and HTM." in SOSP. 2015.  
[R5]. Mitchell, Christopher, et al. "Using One-Sided RDMA Reads to Build a Fast, CPU-Efﬁcient Key-Value Store." in ATC. 2013.  
[R6]. Dragojević, Aleksandar, et al. "FaRM: Fast remote memory." in NSDI. 2014.  
[R7]. Wang, Yuchen, et al. "Dynamically Configuring LRU Replacement Policy in Redis." In MEMSYS. 2020.  
[R8]. Yan, Bin, et al. "Patronus: High-Performance and Protective Remote Memory." in FAST. 2023.  
[R9]. Heo, Taekyung, et al. "Hardware-assisted trusted memory disaggregation for secure far memory." arXiv preprint arXiv:2108.11507 (2021).  

==> revision-plan.tex <==
Dear Dr. Marcos K. Aguilera,

Thanks for shepherding our paper #70, “Anole: An Elastic and Adaptive Memory-Disaggregated Caching System”. We drew up a revision plan based on the reviewers’ comments, as shown in the following. Please let us know if you have new comments or suggestions. We will send you our revised paper by 28th August.

Comment 1: Remove claims about no migration needed. (Q4, Q12) 
Revision: We will remove the claim and explain that using DM can greatly reduce the frequency of data migration for in-memory caching systems in Sections 1 and 2.

Comment 2: Discuss write performance.
Revision: We will discuss the write performance of Anole compared with Redis and CliqueMap in Section 5.

Comment 3: Discuss the separate scaling of application, compute, and memory. (Q1, Q5)
Revision: We will clarify in Sections 2 and 4 how applications use Anole and how applications can independently adjust Anole's compute and memory resources.

Comment 4: Clarify evaluation experiments, baselines, and results per reviewer comments.
Revision: We will clarify our experiment settings in Section 5. Specifically, we will clarify the following settings according to our reviews:
1) What are the parameter settings of Anole? How are these values selected? (Q13, Q17)
We will explain all our parameter settings and why we choose these values in Section 5.
2) Why did you pick CloudPhysics traces randomly? How did you select traces from Twitter and FIU? Why did you ignore traces with less than 10M requests and truncate traces at 40M? Why YCSB-E and YCSB-F are omitted? (Q18, Q24)
We will explain our trace selection criteria clearer in the paper.
3) Your machine has 72 cores. Why do you use 32 cores in the evaluation? (Q19)
We will explain this setting as we did in our reply to Q19.
4) Why do Sections 5.5 and 5.6 rely almost exclusively on the single webmail trace to show flexibility with different caching algorithms and the impact of Anole’s techniques on performance? Why only use YCSB-C to evaluate the frequency cache? (Q20)
We will first clarify that the experiment in Section 5.5 (Figure 23) is irrelevant to traces. We will then mention in our paper that Anole’s performance is similar on other workloads for experiments in Section 5.6. We will direct readers to refer to the more detailed results in our open-source repository.
5) Why did you use the size of the frequency cache in MB instead of the number of cached objects? (Q21)
We will explain that the size of cache entries in the frequency cache varies with the size of the object ID, and we use size in MB for fair comparisons in Section 5.
6) What are the workloads for Figures 20-22? (Q22,Q23)
We will clarify the workloads in Figures 20-22 in the paper, as in our reply to Q22. (Q25)
7) "We generate 10 million keys with 256-byte key-value pairs." Each thread is generating this?
We will clarify how threads load YCSB workloads in Section 5.

Comment 5: Explain the security and fairness implications of Anole. (Q10, Q11)
Revision: We will add an additional subsection in Section 4 to discuss the security and fairness issues.

Comment 6: Discuss the cost of memory allocation and memory registration. (Q14)
Revision: We will explain the cost of memory allocation and memory registration in Section 5.

Comment 7: Will extra hop or resource contention affect the end-to-end performance of applications? (Q2)
Revision: We will clarify in Section 4 there is no extra hop between applications and Anole.

Comment 7: Shifting work to the client side adds more CPU burden on client CPUs. Will applications and Anole contend for resources, such as CPU? (Q1, Q7)
Revision: We will discuss in Section 5 that using Anole does not cause more CPU contention on applications than existing caching systems, e.g., Redis, as we did in our reply to Q1.

Comment 8: Justify better the baselines. (Q3)
Revision: We will justify why we select these baselines better in Section 5.

Comment 9: What kinds of workloads are particularly challenging for Anole, and how well it perform in the worst case? (Q15)
Revision: We will discuss the performance of Anole under different workloads in Section 5, as we did in our reply to Q15.

Comment 9: How realistic is it to scale the cache memory capacity by adding/removing usable memory on a single MN? What needs to change in Anole’s design to support multiple MNs? (Q16)
Revision: We will clarify that Anole’s design is independent of the lower-level memory pool in Section 4. Also, we will clarify in Section 5 that we use a single MN to simulate the memory pool to evaluate Anole.

Comment 10: In section 5.2, why doesn't throughput double from 5Mops to 10Mops with you double the # of CPUs? (Q26)
Revision: We will explain the reason in Section 5.

Comment 10: In Figure 14, what’s the max throughput of Anole? (Q27)
Revision: We will show the max throughput of Anole in Figure XX in the paper.

Comment 11: In Figures 18, 20, and 21, please show real hit rates. Or tell what this is normalized to and indicate the absolute values for normalization. (Q28)
Revision: We use the hit rates of a baseline approach to normalize other approaches. We will clearly explain which approach is used as baselines in these figures. Since the absolute hit rates of each point in these figures are different, it is impossible to show all the absolute hit rates in the paper. Instead, we will release all the absolute hit rates in our open-source repository and direct interested readers to the repository.

Comment 12: What’s the space overhead for keeping metadata in Anole? (Q29)
Revision: We will clarify the metadata overhead of Anole in Section 4, as we did in our reply to Q29.

Comment 13: In Section 5.2, what do you mean by “tail latency”? (Q30)
Revision: We will use 99th percentile latency in Section 5 instead of tail latency.

Comment 14: Why couldn't use CPUs on the memory pool to do the cache eviction? (Q32)
Revision: We will clarify in Sections 1 and 2 that the compute power in the memory pool is too weak to execute cache eviction that locates on data paths.

Comment 14: The frequency-counter cache sacrifices the accuracy of the eviction selection. (Q34, Q46)
Revision: We will discuss the effect of frequency counter cache in Section 4 and Section 5.

Comment 14: The description of Figure 20 in the paper seems to differ from the caption of the figure. (Q36)
Revision: We will revise the caption of Figure 20 to make it consistent with the description.

Comment 15: Figure 24: What is the baseline upon which the improvement is happening? (Q37)
Revision: We will clarify that in Figure 24, we shows the effectiveness of each technique by gradually disabling these techniques on Anole and explain that the improvement is calculated as the throughput deduction of disabling a technique divided by the throughput after disabling the technique.

Comment 16: Figure 5(b): The x-axis ranges up to 512 clients but the text below mentions up to 256. (Q38)
Revision: We will fix the typo in the text.

Comment 17: Can you please clarify and discuss the possible tradeoffs of using different values of l for FIFO eviction history? (Q39)
Revision: We will explain the tradeoffs of using different values for l in Section 4.

Comment 18: What's the bottleneck resource for Anole in Figures 14 and 17? (Q40)
Revision: We will discuss the bottleneck resource for Anole in Section 5.

Comment 18: In Figure 15(a), why CM-LRU has a competitive performance with Anole? (Q41)
Revision: We will explain in Section 5 that the overall throughputs of all these approaches are bounded by their hit rates in the webmail workload. CM-LRU has comparable performance with Anole since their hit rates are closer.

Comment 19: Does the use of last_ts in LRU-K affects the execution of other caching algorithms that depends on last_ts? (Q42)
Revision: We will explain in Section 4 that we fall back to recording the modified timestamp of LRU-K together with cached objects if LRU-K needs to execute with other caching algorithms that rely on last_ts.

Comment 20: Please provide an example of a replacement algorithm that keeps additional metadata with objects, how update() and priority() functions access it, and how GET/SET deals with this additional metadata stored with the object. (Q43)
Revision: We will clarify this in Section 4, as we did in our reply to Q43.

Comment 21: Why latency and cost are client-local information? (Q44)
Revision: We will clarify in Section 4 that we assume the latency and cost of objects are approximately the same among clients and can be estimated based on the object size and the latency/cost of accessing other objects.

Comment 22: Is the size of objects measured in a larger block granularity? (Q45)
Revision: We will explain in Section 4 how Anole measures object sizes with an 8-byte len field, as we did in our reply to Q45.

Comment 23: Why use 0xF to indicate history slots? Why not just use 0? (Q47)
Revision: We will fix the typo in Section 4 and clarify that we use 0xFF to indicate history slots.

Comment 24: It is unclear what information is used by the algorithms in Table 3/Figure 23. (Q48)
Revision: We will clarify the information used by each caching algorithm in Table 3 of the paper.

Comment 25: For Shard-LRU, “It maintains lock-protected LRU lists on the client side with one-sided RDMA verbs.” Should this say “on the server side?” (Q49)
Revision: We will rectify this sentence to “Clients maintain lock-protected LRU lists in the memory pool with one-sided RDMA verbs”.

Q6, Q8, Q9, Q33, Q35, 
Apart from all of the above comments, we will fix all the typos pointed out by reviewers and carefully proofread the final version of the paper.


Best regards,
Jiacheng


==> sosp-rebuttal.tex <==
Thank you for the constructive comments. We address the major concerns in the "Major Questions" section. We answer other questions in the "Other Questions" section.

# Major Questions 
## Review A
**Q1:** Where do applications run? If they run at compute nodes (CNs), will applications and Anole contend for resources, such as CPU?  
**Reply:** Applications run on CNs of the disaggregated memory (DM) architecture. Specifically, we follow the architecture of Google's CliqueMap [62] and FUSEE [61], where each application on a CN exclusively owns a local Anole client as a Linux subprocess on the same CN. Each Anole client has multiple threads on dedicated cores configurable by its owning application. Applications communicate with local Anole clients with shared memory, which has low communication overheads. We will clarify the settings in the paper.  
For the second question, yes, we need to assign additional CPU cores to standalone Anole clients on CNs where applications execute. However, such settings will not add additional resource contention compared with applications using other standalone caching services, *e.g.*, Redis. Specifically, in the experiment of Figure 13, Anole clients with 32 cores on a CN generate higher throughput than Redis clients that consume 36.3 cores out of the 128 assigned CPU cores on two CNs. Anole clients have similar CPU overhead on CNs with Redis clients because the Redis client library spends CPU cycles to encapsulate and decapsulate requests and data according to the Redis communication protocol and network protocols. We will supplement the client-side CPU utilization in the paper.

**Q2:** Will extra hop or resource contention affect the end-to-end performance of applications? How about the end-to-end benefits of applications?  
**Reply:** Since applications communicate with Anole clients with local shared memory, there is no extra hop on the data path when applications use Anole. As for the resource contention on CNs, Anole has client-side computation costs similar to Redis (Q1). Therefore, they do not affect the end-to-end performance of applications.  
Moreover, in our evaluation, we use workloads from real-world applications, including IBM Cloud Object Storage, CloudPhysics, Twitter, and FIU. We believe that evaluating the performance of Anole under these real-world application workloads can reflect the end-to-end benefits of applications using Anole. Such evaluation method is also widely used in other caching work, *e.g.*, CliqueMap [62] and MemC3 [23].

**Q3:** Justify better the baselines.  
**Reply:** We tried our best to find as better baselines as possible. We choose Redis, CliqueMap, and Shard-LRU based on the following considerations. First, to show the elasticity of Anole, we choose Redis, one of the most widely adopted in-memory caching systems that support dynamic resource scaling. Second, to show the efficiency of the cache eviction of Anole on DM, we use CliqueMap, the state-of-the-art RDMA-based key-value caching system deployed in Google. Finally, to show the effectiveness of the sample-based caching framework we designed in Anole, we use Shard-LRU, a straightforward implementation of caching systems on DM.  
To compare Anole with Redis and CliqueMap in a fair manner, we disable their irrelevant features, *e.g.*, replication and persistence. Moreover, we evaluate Redis with its cluster mode so that the performance of Redis is not bounded by a single CPU core. Considering that both Redis and CliqueMap require powerful CPUs to perform well, we compare the performance of Anole, Redis, and CliqueMap with an increasing number of CPU cores on the memory node (MN) in Figure 17. Our evaluation results show that Anole outperforms the two baselines even if they have enough CPU cores on the MN to process requests.

**Q4:** What if the MN runs out of bandwidth in a read-only workload? ... I don't believe Anole (or memory disaggregation in general) can avoid data migration in every scenario, as the paper suggests.  
**Reply:** Your comment is insightful. Yes, we cannot avoid data migration in every scenario. Similar to existing approaches [32,82], Anole relies on a lower-level memory pool to distribute and move data among MNs. Data needs to be migrated by the memory pool when the bandwidth of an MN meets the bottleneck. However, the frequency of data migration in the memory pool is significantly lower than that of Redis. As we discussed in Section 2, Redis needs to migrate data whenever applications need to expand/reduce cache sizes or compute powers. In contrast, Anole does not need to move data when expanding/reducing cache sizes since the cached data is flexibly allocated from the entire memory pool. Moreover, the network bandwidths of modern RNICs on MNs are less likely to be saturated than a single-threaded Redis instance due to their high network bandwidths [73]. Besides, Anole can benefit from existing techniques in the implementation of the memory pool to achieve load balancing [18] and transparent data migration [36]. We will clarify this in the paper.

## Review B
**Q5:** How can the management of caching (compute) be independently scaled against cached data? Aren't you now bundling cache management with client computation?  
**Reply:** For the first question, as discussed in Q1, Anole clients are standalone subprocesses that are colocated with applications on the same CNs. An application can freely scale compute resources by adding or removing the number of CPU cores and the threads of its standalone Anole client on demand. The adjustment of compute resources is independent against cached data because the cached data are stored in the remote memory pool and there is no need to increase or decrease the cache size (memory resources) or move data when adding or reducing CPU cores.   
For the second question, the cache management of Anole is not bundled with client computation since, as we explained in the previous question, applications can freely adjust compute resources of the standalone Anole clients.

**Q6:** My biggest concern is the disconnection between the paper's motivation and what is actually implemented and evaluated.  
**Reply:** There is no disconnection between the paper's motivation and what is implemented. Anole is motivated to address the elasticity issues of existing in-memory caching systems, where their compute and memory resources have to be adjusted together and data have to be migrated whenever resources are adjusted. Our idea is to disaggregate the compute and memory resources of in-memory caching systems to provide better elasticity. Our design and implementation follow the architecture of existing memory-disaggregated systems where applications colocate with clients of the systems on the same CNs (Q1), which allows independent adjustments of compute and memory resources. The design of Anole, *i.e.*, the client-centric caching framework and the distributed adaptive caching scheme, addresses the challenges of executing caching algorithms and adapting to changing compute and memory resources under this architecture. Finally, we evaluated the elasticity, efficiency, and adaptivity of Anole by comparing it with Redis, CliqueMap, and Shard-LRU under various real-world key-value traces.

**Q7:** Shifting work to the client side adds more CPU burden on client CPUs.  
**Reply:** The CPU burden of Anole clients on the client side is similar to that of Redis clients. Please refer to our reply to Q1.

**Q8:** There is no result showing independent scaling of compute and memory. The only one on elasticity is Section 5.2 and Figure 13. But the compute and memory are scaled dependently.  
**Reply:** We understand your concerns that the evaluation of independent scaling of compute and memory is critical to Anole. We have actually studied the performance of Anole when it independently scales compute and memory resources in Figures 13, 20-22. First, in Figure 13, we would like to clarify that the compute and memory are scaled *independently* rather than *dependently*. Specifically, the middle and bottom curves in Figure 13 show the result of two independent experiments. For the middle curve (the red one), we keep the memory size constant and independently increase the number of CPU cores from 32 to 64 and then reduce it from 64 to 32. For the bottom curve (the yellow one), we keep the number of CPU cores constant and independently increase the memory size from 32GB to 64GB and then reduce it from 64GB to 32GB. Moreover, Figures 20 and 21 show the relative hit rates of Anole with fixed memory and varying numbers of CPU cores. Figure 22 shows the hit rate of Anole with a fixed number of CPU cores and varying memory spaces. In conclusion, our results show that Anole can independently scale compute and memory resources.

**Q9:** The evaluation also lacks performance breakdown and thus cannot explain where the performance gain comes from. How much is from the sampling design? The logical FIFO queue design? From using a MAB-based ML prediction? or something else?  
**Reply:** We agree that the performance breakdown of Anole is important to understanding the techniques proposed in this paper. We have actually evaluated the performance breakdown of Anole in Figure 24. In Figure 24, we show the performance of Anole when gradually disabling each technique in Anole, *i.e.*, the frequency-counter cache, the lightweight eviction history (the logical FIFO queue), the lazy weight update scheme, and the sample-friendly hash table. Moreover, Figure 14 shows the performance gain of the sample-based approach against Shard-LRU and Figures 18-22 show the performance gain of the adaptive caching (MAB-based ML prediction) against Anole-LRU and Anole-LFU. In conclusion, we have shown via comprehensive experiments that the mechanisms in Anole design are effective.

## Review C
**Q10:** As clients are actively influencing cache management at the server, can there not be security implications? How do you guarantee that all clients use the same priority functions?    
**Reply:** As discussed in Q1, Anole clients are deployed as subprocesses on CNs. Protecting a process from being maliciously manipulated is orthogonal to the scope of this paper. We can use existing software security techniques, *e.g.*, control-flow integrity (CFI) [R1], to protect Anole clients from being manipulated by applications. For the second question, the candidate priority functions are statically configured in Anole clients and cannot be dynamically modified. Since CFI ensures that applications cannot manipulate Anole client processes, applications must use the same priority functions as statically configured in Anole. We will discuss the security issues in the paper.

**Q11:** Could there not be cases where particular clients are disproportionally disadvantaged? Could not a client manipulate the cache framework so that it is disproportionately advantaged or other (particular) clients are disadvantaged?  
**Reply:** We agree that it is critical to ensure applications to share the cache space in a fair manner. We can employ the expected delaying technique in FairRide [R2] on standalone Anole clients to ensure that applications fairly share the cache. We will discuss the fairness issues in the paper.

## Review D
**Q12:** As individual MNs are still bounded by the throughput limits of their RNICs and memory buses, adding more MNs should still require data rebalancing across MNs.  
**Reply:** Yes, there are cases we do need to migrate data among MNs. However, compared with Redis, the frequency of migrating data is significantly lower. Please refer to our reply to Q4. 

**Q13:** How did you come up with the number 5 and what is the impact of different values of K?  
**Reply:** We choose to sample 5 objects because it is the default value of Redis. A larger K can make the hit rate of the sample-based approximation of a caching algorithm in Anole closer to the precise implementation of the caching algorithm.

**Q14:** The impact of MN controller and the impact of registering RDMA-accessible memory on MN NIC.  
**Reply:** First, we did not pre-allocate remote memory in the memory pool for Anole clients. In our experiments, clients dynamically allocate and free memory spaces from MNs. Hence, we did not underestimate the dynamic memory allocation costs in our experiments. Second, there is no overhead in registering RDMA memory regions when clients dynamically allocate or free memory spaces because MNs are dedicated to remote memory accesses and we pre-register all memory of MNs to their local RNICs on initialization. We will clarify these issues in the paper.

## Review E
**Q15:** What kinds of workloads are particularly challenging for Anole, and how well does it perform in the worst case?  
**Reply:** To the best of our knowledge, no workload that we are aware of is particularly challenging for Anole. Anole is a caching framework on DM where various caching algorithms can be integrated into it and Anole can adaptively select the best one according to the resource and workload changes. Similar to existing adaptive caching approaches [55,68], the performance of Anole on a particular workload largely depends on the candidate caching algorithms configured by users. As we discussed in Section 5, the performance of Anole lies between the candidate caching algorithms on stable workloads and can outperform these candidates on changing workloads or changing resource settings, which is also indicated in our experimental results.

**Q16:** How realistic is it to scale the cache memory capacity by adding/removing usable memory on a single MN? What needs to change in Anole's design to support multiple MNs?  
**Reply:** Anole is not designed for a single MN. In our evaluation, we use a single MN to simulate the memory pool. The design of Anole is agnostic to the implementation of the lower-level memory pool. No modifications are required for Anole to support a memory pool with multiple MNs, as long as the memory pool provides the ALLOC, FREE, READ, WRITE, ATOMIC\_CAS, and ATOMIC\_FAA interfaces, as we have discussed in Section 2.2.

## Questions about experiment settings.
**Q17 (Reviews C&D&E):** Parameters of Anole and Shard-LRU:  
**Reply:**   
|**Anole parameters**|Values|
|--------------------|------|
|#Samples|5|
|#FIFO history entries|Cache size (calculated as the number of objects Anole can store)|
|Batch size of weight update|100|
|Learning rate|0.1|
|FC threshold t|10|
|FC size|10MB|

|**Shard-LRU parameters**|Values|
|------------------------|------|
|#LRU shards|32|
|Lock-fail backoff time|5us|

The number of samples is set according to the default value of Redis. The number of recorded FIFO history entries is set according to the default value of LeCaR [68]. For other parameters, we conducted a grid search and used the best settings for Anole and Shard-LRU. We will clarify all the parameter settings clearer in the paper.

**Q18 (Reviews A&C&E):** Why did you pick CloudPhysics traces randomly? How did you select traces from Twitter and FIU? Why did you ignore traces with less than 10M requests and truncate traces at 40M?  
**Reply:**  First, we did not intentionally select specific traces to show the performance of Anole. In our experiments, we evaluated the performance of Anole on 42 different traces (YCSB\*4, IBM\*23, CloudPhysics\*10, Twitter\*3, Webmail\*1, Changing\*1) of different use cases, *i.e.*, block IO, KV cache on different clusters, and object-store. We randomly use traces to accelerate our evaluation to show the performance of Anole in different use cases. Specifically, for CloudPhysics, we use the first 10 traces. For Twitter, we randomly use 3 traces from the compute, storage, and transient clusters of Twitter as the representatives, and for FIU, we use the webmail trace as it is also selected as a representative trace in Cacheus [55]. Second, we ignore traces with less than 10M requests because they contain too few unique objects. We truncate traces at 40M because the memory capacity of our CNs cannot afford 32 clients to load the entire trace. The design of Anole is agnostic to the workload type or the trace size. We will clarify our trace selection and sizes of traces clearer in the paper. 

**Q19 (Reviews A&C):** Your machine has 72 cores. Why do you only use 32 cores in the evaluation?  
**Reply:** There are two NUMA nodes on each machine and the RNIC is connected to one of the NUMA nodes. We use CPU cores that locate on the same NUMA node as the RNIC (36 cores) and choose 32 for ease of management (multiplies of 8).

**Q20 (Review E):** Why do Sections 5.5 and 5.6 rely almost exclusively on the single webmail trace to show flexibility with different caching algorithms and the impact of Anole's techniques on performance? Why only use YCSB-C to evaluate the frequency cache?  
**Reply:** The experiment of Section 5.5 (Figure 23) is irrelevant to traces. We use webmail to show that Anole can integrate various caching algorithms and these algorithms work in real-world traces. As for the experiments in Section 5.6 (Figures 24-25), Anole performs similarly on other workloads. We only show the results of webmail and YCSB-C due to the space limit. We will clarify this in the paper and release the remaining results in our open-source repository.

**Q21 (Review E):** Why did you use the size of the cache in MB instead of the number of cached entries to show the FC cache size?  
**Reply:** The size of the FC cache is given in MB because the size of an FC cache entry is related to the length of the object ID. For fairness considerations, we limit the size of the FC cache in bytes rather than in the number of cached entries.

**Q22 (Reviews C&E):** What are the workloads for Figures 20-22?  
**Reply:** The workloads of Figures 20-22 are the webmail workload from FIU, which is the same as that of Figures 3, 4, and 5(b) in Section 2. We use the same workload as the previous figures in Section 2 because we are doing the same experiment in these Figures to show the adaptivity of Anole. Particularly, in Figures 3 and 20, we use the webmail of day 7 and day 12, which are LRU and LFU-friendly workloads, respectively. For other Figures (15(a), 16(a), 21, 22, 23, 24), we merge all webmail traces (in different days) as the webmail workload. We will clarify the settings in the paper.

**Q23 (Review E):** Are all clients in Figure 21 running webmail?  
**Reply:** Yes, all clients in Figure 21 run the webmail workload. 

**Q24 (Reviews C&E):** Why YCSB-E and YCSB-F are omitted?  
**Reply:** YCSB-E evaluates the scan performance of tree-based key-value stores and YCSB-F evaluates the performance of transactional read-modify-write operations. These two workloads are skipped since Anole is a hash-table-based caching system that does not support scan and transactional read-modify-write operations.

**Q25: (Review C)** "We generate 10 million keys with 256-byte key-value pairs." Each thread is generating this?   
**Reply:** No, we pre-generate 10 million 256-byte key-value pairs. Threads insert their partitions of keys into Anole according to the total number of threads and their thread IDs. The YCSB workloads are executed after the insertion of keys. 

# Other Questions
## Review A
**Q26:** In Section 5.2, why doesn't throughput double from 5Mops to 10Mops when you double the # of CPUs?  
**Reply:** This is caused by the additional overhead of coroutine scheduling on the added machine.

**Q27:** In Figure 14, what's the max throughput of Anole?  
**Reply:** The max throughput of YCSB-A, YCSB-B, YCSB-C, and YCSB-D are 10.55Mops, 13.09Mops, 13.24Mops, and 13.02Mops, respectively.

**Q28:** In Figures 18, 20, and 21, please show real hit rates, not relative ones. Or tell what this is normalized to (what 1.0 represents?) and indicate the absolute values for normalization.  
**Reply:** Figure 18 is normalized over the hit rates of Random eviction. Figures 20 and 21 are normalized over the hit rates of Anole-LRU. We will clarify the absolute values for normalization in the paper.

**Q29:** What's the space overhead for keeping metadata in Anole?  
**Reply:** The metadata overhead is $80 \cdot C + 4 \cdot N$ bytes, where $C$ is the cache size (calculated as the number of objects Anole can store) and $N$ is the number of experts (candidate caching algorithms) for the distributed adaptive caching. The metadata consist of history entries, the metadata for cached objects, and global expert weights. First, each history entry uses 40 bytes and the total number of recorded history entries is set to be the cache size according to LeCaR [68]. Second, for each cached object, the metadata overhead is 40 bytes (8 bytes for the hash slot and 32 bytes for the access information, as shown in Figure 7). Finally, for each expert, a 4-byte float value is required as its global expert weight.

**Q30:** In Section 5.2, what do you mean by "tail latency"?  
**Reply:** We use 99th percentile latency as tail latency for all our experiments. We will clarify this in the paper.

## Review C
**Q31:** How are Figures 3 and 5(b) different?  
**Reply:** Figure 3 shows how the compute resources assigned to applications with different access patterns affects hit rates. Figure 5(b) shows how the number of concurrent clients executing the same workload affects hit rates. They both show that the caching algorithm with a better cache hit rate changes with varying compute resources.

**Q32:** Why couldn't use CPUs on the memory pool to do the cache eviction?  
**Reply:** As introduced in Section 2.2, MNs in the disaggregated memory pool only have 1-2 weak CPU cores to do management tasks on the control path. However, the cache eviction locates on the data path since *Set* operations have to be blocked until enough spaces are evicted. Relying on these weak CPU cores to do cache eviction will result in poor performance.

**Q33:** Table 1 shows many more fields, while Figure 7 shows only three of these fields. Is three enough? Can there not be more than three?  
**Reply:** As discussed in Section 4.2.1, we find that only access information that is global information needs to be maintained in the hash table. Hence, in the hash table, we record 4 global information, *i.e.*, size, insert\_ts, last\_ts, and freq. Among them, the size information is recorded as the len field in the Atomic Field in Figure 7. For the second question, we discussed in Section 4.2.1 that Anole can extend more access information by storing them together with cached objects. 

**Q34:** The frequency-counter cache sacrifices the accuracy of the eviction selection.  
**Reply:** The threshold t of the frequency-counter cache is set to 10 in our experiment. Using t=10 does not affect the hit rate much, as indicated by the superior hit rates of Anole in our experiments.

**Q35:** Figure 13 results are for one CN? How are you getting 64 cores on the CN?  
**Reply:** Figure 13 results are generated with 1 MN and 2 CNs. 

**Q36:** The description of Figure 20 in the paper seems to differ from the caption of the figure.  
**Reply:** The description in the paper is more accurate. We will make the caption consistent with the description in the paper.

**Q37:** Figure 24: What is the baseline upon which the improvement is happening?  
**Reply:** We'd like to clarify that in Figure 24, we show the effectiveness of each technique by gradually disabling these techniques on Anole. For example, the "-LWU" bar shows the performance of Anole without FC and LWU. Hence, the improvement percentage in the paper is calculated as the throughput deduction of disabling a technique divided by the throughput after disabling the technique. For example, the throughput improvement of the sample-friendly hash table is calculated as $(Tpt_{-LWH} - Tpt_{-SFHT}) / Tpt_{-SFHT}$, where $Tpt_{-LWH}$ indicates the throughput of -LWH in Figure 24. We will clarify this in the paper.

## Review D
**Q38:** Fig. 5(b): The x-axis ranges up to 512 clients but the text below mentions up to 256.  
**Reply:** Thank you for pointing out the mistake. The x-axis is correct. We will fix the typo in the paper.

**Q39:** Can you please clarify and discuss the possible tradeoffs of using different values for l (FIFO history size)?  
**Reply:** Setting a smaller value for l can cause fewer penalties collected by the MAB-based learning algorithm and will make the adaption of caching algorithms slower. On the other hand, setting a larger value for l results in higher storage overhead of recording history entries. We will clarify this in the paper.

**Q40:** What is the bottleneck resource for Anole in Figures 14 and 17?  
**Reply:** The bottleneck resource is the message rate of the RNIC on the MN.

**Q41:** In Figure 15(a), why CM-LRU has a competitive performance with Anole?  
**Reply:** As shown in Figure 16(a), the overall throughputs of all these systems are bounded by their hit rates in the webmail workload. Since the hit rate of CM-LRU is closer to Anole, their performance is comparable.

## Review E
**Q42:** Does the use of last\_ts of LRU-K affects the execution of other caching algorithms that depends on last\_ts?  
**Reply:** If caching algorithms that depend on last\_ts need to cooperate with LRU-K, we fall back to recording the modified timestamp as extended metadata and storing it together with objects to implement LRU-K. We will clarify this in the paper.

**Q43:** Please provide an example of a replacement algorithm that keeps additional metadata with the object, how update() and priority() functions access it, and how GET/SET deals with this additional metadata stored with the object.  
**Reply:** In this case, the extended metadata are stored as a metadata header ahead of each object. The update() and priority() functions take all metadata as input (including default ones in the hash table and the extended ones stored with objects) and call user-defined metadata update and priority calculation functions to deal with the extended metadata. GET/SET operations need to issue an additional RDMA operation to update the metadata stored together with objects. On eviction, additional RDMA\_READs are required to fetch the metadata headers. We will clarify this in the paper.

**Q44:** Why *latency* and *cost* are client-local information?  
**Reply:** We assume that the latency and cost of objects are approximately the same among clients and can be estimated based on the object size and the latency/cost of accessing other objects. We will clarify this in the paper.

**Q45:** Is the size of objects measured in a larger block granularity?  
**Reply:** Yes, we measure the size of objects similar to RACE hashing [82]. Specifically, the size is measured in 64B. For objects larger than $(2^{8}-1) \cdot$ 64B (the len field is 8 bit and we use 0xFF to indicate history entries), Anole stores the remaining object in a second memory block that links to the first one.

**Q46:** If each client can buffer up to t object accesses locally before updating the metadata at the memory node, it seems like the access information could get quite badly out-of-date.  
**Reply:** Anole only buffers the freq field locally instead of the entire access information. The threshold t is set to 10 in our experiments. Using t=10 does not affect the hit rate much, as indicated by the superior hit rates of Anole in our experiments.

**Q47:** Why use 0xF to indicate history slots? Why not just use 0?  
**Reply:** Thank you for your careful review. There is a typo. We use 0xFF instead of 0xF to mark history entries. We cannot simply use 0 because we need to use len=0 to examine whether a slot is empty or not. We will fix the typo in the paper.

**Q48:** It is unclear what information is used by the algorithms in Table 3 / Figure 23.  
**Reply:** We implement these caching algorithms according to [51,8], which introduce their involved access information. We will clarify the information used by each caching algorithm in Table 3.

**Q49:** For Shard-LRU, "It maintains lock-protected LRU lists on the client side with one-sided RDMA verbs." Should this say "on the server side"?  
**Reply:** Yes, the sharded LRU lists are stored on the MN and maintained concurrently by all clients. We will clarify this in the paper.


[R1]. https://clang.llvm.org/docs/ControlFlowIntegrity.html  
[R2]. Pu, Qifan, et al. "FairRide: Near-Optimal, fair cache sharing." NSDI, 2016.

